Emergence and Evolution of Hierarchical Structure in Complex Systems

It is well known that many complex systems, both in technology and nature, exhibit hierarchical modularity: smaller modules, each of them providing a certain function, are used within larger modules that perform more complex functions. What is not well understood however is how this hierarchical structure (which is fundamentally a network property) emerges, and how it evolves over time. We propose a modeling framework, referred to as Evo-Lexis, that provides insight to some fundamental questions about evolving hierarchical systems. Evo-Lexis models the most elementary modules of the system as symbols ("sources") and the modules at the highest level of the hierarchy as sequences of those symbols ("targets"). Evo-Lexis computes the optimized adjustment of a given hierarchy when the set of targets changes over time by additions and removals (a process referred to as "incremental design"). In this paper we use computation modeling to show that: - Low-cost and deep hierarchies emerge when the population of target sequences evolves through tinkering and mutation. - Strong selection on the cost of new candidate targets results in reuse of more complex (longer) nodes in an optimized hierarchy. - The bias towards reuse of complex nodes results in an "hourglass architecture" (i.e., few intermediate nodes that cover almost all source-target paths). - With such bias, the core nodes are conserved for relatively long time periods although still being vulnerable to major transitions and punctuated equilibria. - Finally, we analyze the differences in terms of cost and structure between incrementally designed hierarchies and the corresponding "clean-slate" hierarchies which result when the system is designed from scratch after a change.

==> 02-related-work1.tex <==
% \section{Related Work}
\section{\color{red} Discussion and Prior Work}
\label{evolexis-related}
% Constantine's note: we may need to move this section in the Discussion section. The reader will have a better idea about our approach and results by then. 

% Note: I have written a related work write-up before and I'm including the compiled pdf in the project folder. Here, I just mention the main themes which of course should be trimmed down.

\ps{Evo-Lexis is an attempt for investigating the properties of hierarchically modular systems. We find Evo-Lexis to be primarily related to three main themes of research: first, the properties of modularity and hierarchy and the research on their origins in complex systems; second, 
the hourglass property; and lastly, the interplay between design optimality and evolution.}

\subsection{Modularity and Hierarchy}
% Modularity and hierarchy almost seem to be tied together to the extent that it is impossible to think of one without considering the other. 
\ps{It is observed in the mechanism of our framework that the targets in the Lexis-DAG should evolve in certain ways (through partial mutations, recombinations, etc.) so that smaller substrings (i.e. sub-modules in a bigger picture) can arise in a Lexis-DAG.} ``Modularly Varying Goals'' have been shown to contribute to the emergence of modularity. In particular, Kashtan and Alon \cite{kashtan2005, kashtan2007}, motivated by the presence of modularity and  hierarchy in biological networks, have proposed  an explanation for the appearance of modular network motifs. By applying modular changes to logic circuits and evolving neural networks for pattern recognition tasks, they show that modularity in the goals (what we refer to as ``targets'') leads to the emergence of modularity in the organization of the system, whereas randomly varying goals do not lead to modular architectures.

\ps{In another line of, it seems the existence of modularity and hierarchy is very often followed when cost optimization is a driver in the goal or design of the system. Since, the presented framework in our research comprises all of these aspects (modularity, hierarchy and optimization), we review the related literature to see what origins are considered for these patterns and what similarities and difference hold between our work and other's models.} Clune et al. show that modularity is a key driver for the evolvability of complex systems \cite{clune2012}. The authors demonstrate that selection mechanisms that minimize the cost of connections between nodes in a networked system result in a modular architecture. This is shown by evolving networks that solve pattern recognition tasks and Boolean logic tasks. The inputs sense the environment (e.g. pixels) and produce outputs in a feed-forward manner (e.g. the existence of pattern of interest). In other words, the networks that have evolved for optimizing both performance (accuracy in recognition) and cost (network connections) are more modular and evolvable (in the sense of being adaptable to new tasks) than those optimized for performance only. In a follow-up study by Mengistu et al. in \cite{clune2016}, it is shown that the minimization of the cost of connections also promotes the evolution of hierarchy, the recursive composition of sub-modules. When not modeling the cost of connections, even for tasks with hierarchical structure (e.g. a nested boolean function), a hierarchical structure does not emerge.



\ps{More broadly on the topic of modularity and hierarchy, there are further specific modeling and also real evidence of modularity and combinatorial nature of the real systems.} Arthur et al. model the combinatorial nature of technology using logic circuit gates \cite{arthur2006}. Each designed element is a combination of simpler existing elements. Their simulation model results in a modularly organized system, in which complex functions are only possible by first creating simpler ones as building blocks. 
% The results are also important in terms of the fact that there have been shown equivalent results in biological evolution. 
In \cite{youn2015}, a study of USPTO data gives evidence for the combinatorial evolution of technology. The authors find that the rate of new technological capabilities is slowing down, but that a huge number of combinations allows for a ``practically infinite space of technological configurations''. By considering technology as a combinatorial process, \cite{kim2016} uses USPTO data to investigate the extent of novelty in patents. They propose a likelihood model for assessing the novelty of combinations of patent codes. Their results show that patents are becoming more conventional (rather than novel) with occasional novel combinations.


\subsection{Hourglass Property} 
A property of many hierarchical networks is the \emph{hourglass effect}, which means that the system starts from many inputs and produces many outputs through a relatively small number of intermediate modules that are critical for the operation of the entire system \cite{sabrin2016}. \ps{This property is one of the main themes investigated in our work and we find our results to be complementary and in line with prior work in this area.}

Akhshabi et al. studied the \emph{developmental hourglass} which is the pattern of increasing morphological divergence towards earlier and later embryonic development \cite{akhshabi2014}. The authors conclude that 
the main factor that drives the emergence of the hourglass architecture in that context is that the developmental gene regulatory networks become increasingly more specific, and thus sparser, as developmemt progresses.
% i.e. the specificity of  these layers should be increasing.

Earlier, the same authors in \cite{akhshabi2011} were inspired by the hourglass-resemblence of the Internet protocol stack in which the lower and higher layers tend to see frequent innovations, while the protocols at the waist of the hourglass appear to be ``ossified''. The authors present an abstract model, called \emph{EvoArch}, to explain the survival of popular protocols at the waist of the protocol stack.  
The protocols which provide the same functionality in each layer compete with each other and, just as in \cite{akhshabi2014}, the increasing specificity and sparsity is what causes the network to have an hourglass architecture.

Friedlander et al. focus on linear layered networks \cite{alon2015} and
show that in such systems the hourglass architecture emerges due to the compressibility of the input-output relation. In their model, this is interpreted as rank-deficiency of the input-output matrix that describes the function of the system. A further requirement is that there should be a tendency to reduce the number of links in the network.

The hourglass effect has been also investigated in general (non-layered) hierarchical dependency networks. The analysis in \cite{sabrin2016} is based on the idea of identifying the core of a dependency network based on the number of source-to-target dependency paths, similar to our study. That framework shows the presence of the hourglass property in various technological, natural and information systems. The authors also present a model called \emph{Reuse-Preference}, capturing the bias of new modules to reuse intermediate modules of similar complexity instead of connecting directly to sources or low complexity modules. 

Despite this previous work, the interplay between the hourglass property and cost optimization in hierarchical networks has not been explored in previous research. In this work, we explore under what conditions the hourglass property emerges in hierarchical optimization-based and incremental design.

\subsection{Interplay of Design Adaptation and Evolution}
A main theme in our study is the interplay between changes in the environment (the targets that the system has to support) and the internal design or architecture of the system. 
% Although not directly related to our work, previously there have been attempts in modeling how design methodologies affect the evolution of technology, and vice versa. 
Bakhshi et al. investigate a network topology design scenario in which the goal is to design a valid communication network between a set of nodes \cite{bakhshi2012}. The authors formulate and compare the consequences of two different optimization scenarios for that goal: \emph{incremental design} in which the modification cost between the two last snapshots of the design is minimized, and \emph{optimized design} in which the total cost of the network is minimized in every increment. Focusing on the case of ring networks, even though the incremental designs are more costly, the relative cost overhead is shown to not increase as the network grows. In a follow-up study, focused on mesh networks, the same observation is made and further, the incremental design is shown to be producing larger density, lower average delay and more robust topologies \cite{bakhshi2013}. \ps{Similar approaches to incremental design have been taken in other design problems as well, for example, in deep neural networks (DNNs) and specifically in how one can ``transfer'' and ``adapt'' the learned features  of a deep network from one task to another \cite{dnn}. Analogous to how new targets are incrementally included in the Lexis-DAG (reusing previously appearing nodes, and then optimizing the DAG over them), learning a new task by a DNN can be re-factored as reuse of ``frozen'' features from a previous similar task and then, ``fine-tuning'' the new network. Improvements in speed and even generalization capability of DNNs is a perfect example of the successful use of incremental approaches in a hierarchically designed system and why it is vastly considered instead of clean-slate methodologies in such systems.
}

\ps{
In terms of algorithmic aspects, the type of incremental design policies that we consider in this paper (which are assumed to be a realization of what happens in natural and technological systems) is categorized under the umbrella of \emph{online algorithms} \cite{online-algs-thesis}: given a sequence of input, the algorithm finds a sequence of solutions that build incrementally while adapting to the changes in the input without knowing the input sequence in advance. One difference that our setting has to the setting of online algorithms is the fact that the past input is removed and newer input is replaced as the time passes. \emph{Competitive analysis} has been the most focused topic of research in the study of online algorithms which is on theoretical comparison of the solution quality of an online algorithms to its offline counterpart (that is when the entire input is available to the algorithm). In this research, we apply a similar experimental analysis in terms of the differences of the cost and the topological metrics of the inferred incremental and clean-slate hierarchies. 
}
% McNerney et al. presents a model on how the cost of a technology evolves \cite{mcnerney2011}. The authors describe an environment, where a technological system is considered to be a clustered composition of smaller components. Innovation or introduction of new components is what drives the design of the system (modeled as a DSM - Design Structure Matrix), as long as the total cost of the cluster is reduced according to predefined criteria. They show that the cost of the  technology and number of innovation attempts follow a power-law relationship.
\subsection{\ps{Implications on the Analysis of Real Data}}
The Evo-Lexis model is certainly a quite general and abstract model and it does not attempt to capture any domain-specific aspects of biological or technological evolution. As such, it makes several assumptions that can be criticized as unrealistic, such as that all targets have the same length, their length stays constant, the fitness of a sequence is strictly based on its hierarchical cost, etc.
We believe that such abstract modeling is still valuable because it can provide insights about the qualitative properties of the resulting hierarchies under different target generation models.
Having said that however, we also believe that the predictions of the Evo-Lexis model should be tested using real data from evolving systems in which the outputs can be well represented by sequences. 

One such system is the iGEM synthetic DNAs dataset \cite{igem}. The target DNA sequences in the iGEM dataset are built from standard ``BioBrick parts'' (more elementary  DNA sequences) that collectively form a library of synthetic DNA sequences. These sequences are submitted to the Registry of Standard Biological Parts in the annual iGEM competition. Previous research in \cite{dnaSynthPaper,siyari2016a} has shown evidence that it is plausible to consider a hierarchical organization for such targets. In the near future, we will investigate how to apply the Evo-Lexis framework in the timeseries of iGEM sequences. We will examine how those sequences deviate from the Evo-Lexis assumptions (e.g., their alphabet changes with time), and whether the resulting hierarchies exhibit the qualitative properties we focused on in this paper.
